Learning to Bid in Repeated First-Price Auctions with Budgets

Budget management strategies in repeated auctions have received growing attention in online advertising markets. However, previous work on budget management in online bidding mainly focused on second-price auctions. The rapid shift from second-price auctions to first-price auctions for online ads in recent years has motivated the challenging question of how to bid in repeated first-price auctions while controlling budgets. In this work, we study the problem of learning in repeated first-price auctions with budgets. We design a dual-based algorithm that can achieve a near-optimal $\widetilde{O}(\sqrt{T})$ regret with full information feedback where the maximum competing bid is always revealed after each auction. We further consider the setting with one-sided information feedback where only the winning bid is revealed after each auction. We show that our modified algorithm can still achieve an $\widetilde{O}(\sqrt{T})$ regret with mild assumptions on the bidder's value distribution. Finally, we complement the theoretical results with numerical experiments to confirm the effectiveness of our budget management policy.

==> Budget + FPA (arxiv)/sections/abstract.tex <==
\begin{abstract}

Budget management strategies in repeated auctions have received growing attention in online advertising markets. However, previous work on budget management in online bidding mainly focused on second-price auctions. The rapid shift from second-price auctions to first-price auctions for online ads in recent years has motivated the challenging question of how to bid in repeated first-price auctions while controlling budgets.

In this work, we study the problem of learning in repeated first-price auctions with budgets. We design a dual-based algorithm that can achieve a near-optimal $\widetilde{O}(\sqrt{T})$ regret with full information feedback where the maximum competing bid is always revealed after each auction. We further consider the setting with one-sided information feedback where only the winning bid is revealed after each auction. We show that our modified algorithm can still achieve an $\widetilde{O}(\sqrt{T})$ regret with mild assumptions on the bidder's value distribution. Finally, we complement the theoretical results with numerical experiments to confirm the effectiveness of our budget management policy.

\end{abstract}

==> Budget + FPA (arxiv)/sections/algorithm-one.tex <==
\subsection{One-sided Information Feedback}
\label{sec: one}

This subsection provides a modified algorithm for the scenario with one-sided information feedback. We show an $\widetilde{O}(\sqrt{T})$ regret can still be achieved with an assumption on the bidder's value distribution.

As the bidder can only observe the highest competing bid $d_s$ after losing at round $s$ under one-sided information feedback, she can no longer estimate the expected rewards and costs in each round using all past rounds as in \Cref{algo: full}. Specifically, given value $v_t$ and bid $b$, if $b < b_s$ and $b_s \geq d_s$, she cannot determine $\bm{1}\{b \geq d_s\}$, so that she cannot calculate $\widetilde{r}_t(v_t, b), \widetilde{c}_t(b)$ as in \eqref{eqn: estimate r full}, \eqref{eqn: estimate c full}. Therefore, we need new estimators for the expected rewards and costs. 

For this purpose, we first discretize the value space into a set of size $M$, $\calV = [v^1, \cdots, v^M]$ with $v^m = (m-1)/M \cdot \bar{v}$, and the bid space into a set of size $K$, $\calB = \{b^1, \cdots, b^K\}$ with $b^k = (k-1)/K \cdot \bar{v}$. Then, we denote by $n_t^k$ the number of observed bids lower than $b^k$ before round $t$:
\begin{align}
    n_t^k \coloneqq \sum_{s=1}^{t-1} \bm{1}\left\{b_s \leq b^k\right\}. \label{eqn: count one}
\end{align}
Given $v^m$ and $b^k$, we define two estimators under one-sided information feedback as
\begin{align}
    \widetilde{r}_t(v^m, b^k) = &\frac{1}{n_t^k}\sum_{s = 1}^{t-1}\bm{1}\left\{b_s \leq b^k\right\}\bm{1}\left\{b^k \geq d_s\right\}\left(v^m - b^k\right), \label{eqn: estimate r one} \\
    \widetilde{c}_t(b^k) = & \frac{1}{n_t^k}\sum_{s = 1}^{t-1}\bm{1}\left\{b_s \leq b^k\right\} \bm{1}\left\{b^k \geq d_s\right\}b^k. \label{eqn: estimate c one}
\end{align}
Note that the equations \eqref{eqn: estimate r one} and \eqref{eqn: estimate c one} are measurable with respect to the available history $\calH_t^O$. If $b_s \geq d_s$, we have $\bm{1}\left\{b_s \leq b^k\right\}\bm{1}\left\{b^k \geq d_s\right\} = \bm{1}\left\{b_s \leq b^k\right\}$; if $b_s \leq d_s$, the bidder can observe the exact $d_s$ to determine $\bm{1}\left\{b^k \geq d_s\right\}$.

Since $(d_s)_{s=1}^{t-1}$ are not mutually independent conditioned on $(b_s)_{s=1}^{t-1}$, $\widetilde{r}_t(v^m, b^k)$ and $\widetilde{c}_t(b^k)$ are actually not unbiased estimators. However, we can still prove via a martingale argument that they approximate well to the expected reward $r(v^m, b^k) = (v^m-b^k)G(b^k)$ and the expected cost $c(b^k) = b^kG(b^k)$ with high probability, which is formalized as the following lemma.

\begin{lemma}
\label{lem: one azuma}
Under \Cref{algo: one}, with probability at least $1-\delta$, we have $\forall t\geq 2, m\in [M], k\in [K]$,
\begin{align}
    |\widetilde{r}_t(v^m, b^k) - r(v^m, b^k)| \leq & \bar{v}\cdot \sqrt{\frac{4 \ln{T}\ln{\left(KT/\delta\right)}}{n_t^k}}, \\
    |\widetilde{c}_t(b^k) - c(b^k)| \leq & \bar{v}\cdot\sqrt{\frac{4 \ln{T}\ln{\left(KT/\delta\right)}}{n_t^k}}.
\end{align}

\end{lemma}

By \Cref{lem: one azuma}, we know that the more bids that are lower than $b^k$, the more accurate the estimation of $r(v^m, b^k)$ and $c(b^k)$. However, bidding low in order to benefit future estimates may cause great loss in the current round. The existence of the budget constraint further increases the difficulty of balancing present and future rewards.

\begin{algorithm}[p]
\caption{Bidding Algorithm for First-Price Auctions with Budgets under One-Sided Information Feedback}\label{algo: one}
\begin{algorithmic}[1]
\setcounter{ALC@unique}{0}
        \STATE {\bfseries Input:} Time horizon $T$; budget $B=\rho T$; 
        value set $\calV = [v^1, \cdots, v^M]$ with $v^m = (m-1)/M \cdot \bar{v}$; 
        bid set $\calB = \{b^1, \cdots, b^K\}$ with $b^k = (k-1)/K \cdot \bar{v}$; 
        update step $\epsilon > 0$; 
        failure probability $\delta\in (0,1)$.
        \STATE {\bfseries Initialization:} The bidder bids $b_1 = 0$ and set $B_2 = B, \lambda_2 = 0$. Set $\calB_0^m \gets \calB$ for each $v_m \in \calV$. \label{algo: one initialization}
        % Active bid set $\calB_{m} \gets \calB$ and minimum count $N_{m}\gets 0$, for each $v_m \in \calV$; all (empirical reward, action count) pairs $(\bar{r}_{0,m,k}^0, n_{0,k})$ initialized to $(0,0)$ for each $v_m \in \calV, b_k \in \calB$; shading parameter $\lambda_1 = 0$.
	\FOR{$t\in\{2,\cdots,T\}$}
        \STATE The bidder receives the value $v_t \in [0,1]$;
        \STATE The bidder counts the observations by \eqref{eqn: count one}, and estimates the rewards and costs  by \eqref{eqn: estimate r one} and \eqref{eqn: estimate c one}. \label{algo: one estimate}
        \FOR{$m\in\{1,2,\cdots,M\}$}
        \STATE The bidder eliminates bids by: \label{algo: one partial order}
        \begin{align}
            \calB_{t-1}^m = \left\{b^k\in \calB_{t-1}^m: b^k \geq \max_{s < m} \inf \calB_t^{s}\right\}.
        \end{align}
        \STATE The bidder computes the confidence bound:
        \begin{align}
            w_t^m = \bar{v}\cdot \sqrt{\frac{4\ln{T}\log(KT/\delta)}{N_t^m}},
        \end{align}
        where $N_t^m = \min_{b^k\in \calB_{t-1}^m} n_t^k$.
        \STATE The bidder eliminates bids by: \label{algo: one high reward bid}
            \begin{align}
                \calB_t^m \gets \Big\{& b^k\in  \calB_{t-1}^m: \widetilde{r}_t(v^m, b^k) \nonumber \\
                \ge & \max_{b^{k'} \in \calB_{t-1}^m}\widetilde{r}_t(v^m, b^{k'}) - 2 w_t^m \Big\}. 
            \end{align}
        \ENDFOR
        \STATE The bidder chooses \label{algo: one value shading}
        \begin{align}
            v^{m(t)} = \max\{u\in \calV: u \leq v_t/(1+\lambda_t)\}.
        \end{align}
        \STATE The bidder submits a bid $b_t = \inf \calB_{t}^{m(t)}$; \label{algo: one bid}
            \STATE The bidder updates the parameter \label{algo: one update}
            \begin{align}
                \lambda_{t+1} = {\rm Proj}_{\lambda > 0} \left(\lambda_t - \epsilon\left(\rho - \widetilde{c}_t(b_t)\right) \right).
            \end{align}
        \STATE The bidder observes $x_t$ and $(1-x_t)d_t$;
        \STATE The bidder update the remaining budget 
        \begin{align}
            B_{t+1} = B_t - c_t.
        \end{align}
        \IF{$B_{t+1} < \bar{v}$}
            \STATE \textbf{break}
        \ENDIF
	\ENDFOR
\end{algorithmic}
\end{algorithm}

We depict our modified algorithm for one-sided information feedback in \cref{algo: one}. The main difference with \Cref{algo: full} is that the bidder maintains an active set of high reward bids for each $m\in [M]$. After observing the value $v_t$ in round $t$, the bidder shades it by $(1+\lambda_t)$ (\Cref{algo: one value shading}) and rounds it to $v^{m(t)}\in \calV$. Then the bidder submits a bid among the active bid set $B^{m(t)}_t$ (\Cref{algo: one bid}).
% Recall that \Cref{algo: full} aims to maximize the cost-adjust reward in each round
The value-shading step essentially aligns the objectives of different rounds. 
Observe that
\begin{align*}
    r(v_t, b^k) - \lambda_t c(b^k) = & \left(v_t - \left(1+\lambda_t\right)b^k\right)G(b^k) \\
    = & (1+\lambda_t) \left(\frac{v_t}{1+\lambda_t} - b^k\right)G(b^k) \\
    = & (1+\lambda_t) \cdot r(v_t/(1+\lambda_t), b^k).
\end{align*}
Thus, with $v^m\approx v_t/(1+\lambda_t)$, maximizing $r(v_t, b) - \lambda_t c(b)$ is approximately equivalent to maximizing the reward $r(v^m, b)$ as if the bidder is participating in a first-price auction without any budget constraint and the value is $v^m$. 

Instead of submitting the bid with the highest estimated reward $\widetilde{r}_t({v^m, b^k})$, the algorithm chooses the smallest bid in $\calB_t^m$ in order to make future estimates as accurate as possible. In addition to filtering bids according to the expected rewards and confidence bounds (\Cref{algo: one high reward bid}), the algorithm also eliminates some small bids from the active sets in \Cref{algo: one partial order}. This elimination increases $N_t^m$ so that the bidder can use smaller confidence bounds to prune the active sets. As long as the best bid for a value $v^m$ remains in the active set $\calB^m_t$, the elimination can further control the regret.

To prove that the best bids are not eliminated, we leverage a special partial order property of first price auctions
% to further control the regret
, i.e., 
$b^*(v) = \arg\max_b (v-b)G(b)$ is non-decreasing in $v$. In particular, for our scenario with discretization, $\widetilde{b}(v) = \arg\max_{b\in \calB} (v-b)G(b)$ is non-decreasing in $v$. The property guarantees that with high probability, $\widetilde{b}(v^m)$, which approximately maximizes $r(v^m, b)$, is not eliminated from the active set $B^m_{t-1}$ by \Cref{algo: one partial order}. (See \Cref{lem: one elimination}.)

% Moreover, with the help of partial order, we can ensures for any $t$, the bidder has submitted enough small bids for the estimates under the following technical assumption required by our analysis.

% In particular, we have the following lemma \Cref{lem: increasing optimal bid} for our scenario with budget constraints.
% \begin{lemma}
% \label{lem: increasing optimal bid}
% Let $b^*(v) = \arg\max_b (v-b)G(b)$ (taking the smallest if there are ties) and $v^{m(t)} = \max\{u\in \calV: u \leq v_t/(1+\lambda_t)\}$. We have
% $$\frac{v_s}{1+\lambda_s} \leq \frac{v_t}{1+\lambda_t} \Longrightarrow b^*(v^{m(s)}) \leq b^*(v^{m(t)}).$$
% \end{lemma}

\begin{assumption}
\label{asm: main}
The cumulative probability distribution $F$ is continuous with bounded density function $f$ satisfying $0 < \underline{f} < f(v) < \overline{f} < \infty$ for $v\in [0, \bar{v}]$.
\end{assumption}

\Cref{asm: main} is a technical assumption required by our analysis. We note that the existence of positive bounds on the density function is a common assumption in various learning problems. For example, \citet{balseiro2019learning} took it as one of the sufficient conditions for the strong convexity of the dual objective function.
% Then, with the help of partial order, we can 

\begin{lemma}
\label{lem: main}
Suppose that \Cref{asm: main} holds. We have
\begin{align*}
    \bbE_{\vv, \vd} \left[\sum_{t=2}^T \sqrt{1\big/N_t^{m(t)}}\right] \leq \widetilde{O}\left(\sqrt{T}\right).
\end{align*}
\end{lemma}

For full information feedback, the estimation error in round $t$ is $O(\sqrt{\ln T/(t-1)})$ by \Cref{lem: full dkw} so that we are able to control the sum of errors within $\widetilde{O}(\sqrt{T})$. \Cref{lem: main} establishes that for one-sided information feedback, we can get a similar result given \Cref{asm: main} holds, which constitutes a key part of the proof of the following \Cref{thm: one}.

\begin{theorem}
\label{thm: one}
Suppose that \Cref{asm: main} holds. For repeated first-price auctions with budget constraints and one-sided information feedback, there exists constants $C_1, C_2, C_3$, such that \Cref{algo: one} can achieve
\begin{align*}
    Reg(\pi) \leq C_1\sqrt{T\ln{(KT^2)}}\ln{T} + C_2\frac{T}{M} + C_3\frac{T}{K}.
\end{align*}
\end{theorem}

Particularly, when choosing $K = M = O(\sqrt{T})$, we obtain that $Reg(\pi) \leq \widetilde{O}(\sqrt{T})$ when $T$ is sufficiently large. We note that to prove \Cref{thm: one}, \Cref{asm: main} is sufficient but may not be necessary. In \Cref{sec: exp}, we run numerical experiments with further discussion.

==> Budget + FPA (arxiv)/sections/algorithm.tex <==
\section{Bidding Algorithms and Analysis}

In this section, we first design and analyze an algorithm for Problem~\eqref{eqn: problem} with full information feedback, which reveals our high-level idea on budget management in repeated first-price auctions. We prove that the algorithm can achieve an $\widetilde{O}(\sqrt{T})$ regret. Then we modify our algorithm to accommodate the setting with only one-sided information feedback by using value shading and leveraging a special partial order property possessed by first-price auctions. The modified algorithm can still achieve an $\widetilde{O}(\sqrt{T})$ regret under mild assumptions. All omitted proofs in this section can be found in the appendix.

\subsection{Full Information Feedback}
\label{sec: full}

Our bidding algorithm for full information feedback is depicted in \Cref{algo: full}. The bidder first conducts a one-round exploration to make an appropriate initialization (\Cref{algo: full initialization}). After observing the value $v_t$ in each round $t=2, \ldots, T$, the bidder constructs estimates of empirical rewards and costs based on all historical observations and submits a bid that maximizes a cost-adjusted reward (\Cref{algo: full value,algo: full estimate,algo: full bid}). Then the bidder updates $\lambda_t$ using the empirical cost of the submitted bid $\widetilde{c}_t(b)$ and her average budget $\rho$ (\Cref{algo: full update}). The variable $\lambda_t$ plays a key role in adjusting the pace at which the bidder depletes her budget. By the choice of $b_t$, we must have $b_t \leq v_t/(1+\lambda_t)$. If the bidder bids too high in past rounds, $\lambda_t$ tends to be larger, thereby controlling the bids in future rounds. 

\begin{algorithm}[t]
    \caption{Bidding Algorithm for First-Price Auctions with Budgets under Full Information Feedback}
    \label{algo: full}
    \begin{algorithmic}[1]
    \setcounter{ALC@unique}{0}
        \STATE {\bfseries Input:} Time horizon $T$; budget $B=\rho T$; update step $\epsilon > 0$; failure probability $\delta > 0$.
        \STATE {\bfseries Initialization:} The bidder bids $b_1 = 0$ and set $B_2 = B, \lambda_2 = 0$. \label{algo: full initialization}
        \FOR{$t\in\{2,\cdots,T\}$}
            \STATE The bidder receives the value $v_t \in [0,\bar{v}]$. \label{algo: full value}
            \STATE The bidder estimates the rewards and costs: \label{algo: full estimate}
            \begin{align}
                \widetilde{r}_t(v_t, b) = & \frac{1}{t-1}\sum_{s = 1}^{t-1}\bm{1}\left\{b \geq d_s\right\}\left(v_t - b\right), \label{eqn: estimate r full}\\
                \widetilde{c}_t(b) = & \frac{1}{t-1}\sum_{s = 1}^{t-1}\bm{1}\left\{b \geq d_s\right\}b. \label{eqn: estimate c full}
            \end{align}
            \STATE The bidder submits a bid: \label{algo: full bid}
            \begin{align}
                b_t \in \arg\max_b \left(\widetilde{r}_t(v_t, b) - \lambda_t \widetilde{c}_t(b)\right). \label{eqn: best b full}
            \end{align}
            (Taking the smallest if there are ties.)
            \STATE The bidder updates the parameter \label{algo: full update}
            \begin{align}
                \lambda_{t+1} = {\rm Proj}_{\lambda > 0} \left(\lambda_t - \epsilon\left(\rho - \widetilde{c}_t(b_t)\right) \right).
            \end{align}
            \STATE The bidder observes the maximum competing bid $d_t$.
            \STATE The bidder update the remaining budget 
            \begin{align}
                B_{t+1} = B_t - c_t.
            \end{align}
            \IF{$B_{t+1} < \bar{v}$}
                \STATE \textbf{break}
            \ENDIF
        \ENDFOR
    \end{algorithmic}
\end{algorithm}

To provide more intuition on the choice of $b_t$ and the update procedure of $\lambda_t$, we consider an alternative optimization problem with a soft budget constraint:
\begin{equation}
\label{eqn: soft problem}
    \begin{aligned}
    \max_{\pi} & \ \bbE^{\pi}_{\vv, \vd} \left[\sum_{t=1}^T \bm{1}\left\{b^{\pi}_{t} \geq d_{t}\right\}\left(v_t - b_t^{\pi}\right)\right] \\
    \text{s.t. } & \ \bbE^{\pi}_{\vv, \vd} \left[\sum_{t=1}^T \bm{1}\left\{b^{\pi}_{t} \geq d_{t}\right\}b^{\pi}_t\right] \leq \rho T.
    \end{aligned}
\end{equation}
The Lagrangian dual objective of Problem~\eqref{eqn: soft problem} is
\begin{align*}
    & \bbE^{\pi}_{\vv, \vd} \left[\sum_{t=1}^T \left(\bm{1}\left\{b^{\pi}_{t} \geq d_{t}\right\}\left(v_t - (1+\lambda)b_t^{\pi}\right) + \lambda\rho\right)\right] \\
    = & \sum_{t=1}^T \left(\bbE^{\pi}_{\calH_t, v_t} \Big[\left(v_t - (1+\lambda)b_t^{\pi}\right)G\left(b^{\pi}_{t}\right)\Big] + \lambda\rho \right),
\end{align*}
where the equality holds since $b_t^{\pi}$ is independent of $d_t$ as well as other future values and maximum competing bids. For a fixed $\lambda$, the dual objective is maximized by bidding $b_t \in \arg\max_b (v_t - (1+\lambda)b)G(b)$, which is irrelevant to the historical observations $\calH_t$. 

We denote by $\Pi_1$ the set of all strategies that satisfy the soft budget constraint in Problem~\eqref{eqn: soft problem}. By weak duality, we have
\begin{align}
    & \max_{\pi \in \Pi_1} R(\pi) \nonumber \\
    \leq & \min_{\lambda\geq 0} T \left(\bbE_{v} \left[\max_b \left(v - (1+\lambda)b\right)G\left(b\right)\right] + \lambda\rho \right). \label{eqn: soft problem upper bound}
\end{align}
Our algorithm adopts an online gradient descent scheme to approximate the right hand side of \eqref{eqn: soft problem upper bound}, which is also an upper bound on the optimal value of Problem~\eqref{eqn: problem} since $\Pi_0 \subseteq \Pi_1$. A crucial challenge here is that the bidder does not know the prior distribution $G$ so she cannot calculate the exact maximum point of $(v - (1+\lambda)b)G(b)$. To deal with this issue, we adopt the distribution estimation method and use $\widetilde{r}_t(v_t, b), \widetilde{c}_t(b)$ in place of $(v-b)G(b), bG(b)$. As $t$ grows, the estimates become more accurate. The following lemma shows that $\forall v_t, b$, $\widetilde{r}_t(v_t, b)$ and $\widetilde{c}_t(b)$ are good estimates of $r(v_t, b) \coloneqq (v_t - b)G(b)$ and $c(b) \coloneqq bG(b)$ respectively. 
\begin{lemma}
\label{lem: full dkw}
Under \Cref{algo: full}, with probability at least $1 - \delta$, we have for all $t \geq 2$ and $b \leq \bar{v}$,
\begin{align}
    |\widetilde{r}_t(v_t, b) - r(v_t, b)| \leq & \bar{v}\cdot \sqrt{\frac{\ln \left(2T/\delta\right)}{2(t-1)}}, \label{eqn: full dkw r} \\
    |\widetilde{c}_t(b) - c(b)| \leq & \bar{v}\cdot \sqrt{\frac{\ln \left(2T/\delta\right)}{2(t-1)}}. \label{eqn: full dkw c}
\end{align}
\end{lemma}
% Here we only need to consider $b \leq \bar{v}$ as the bids above the value are always irrational with or without budget constraints.

\begin{theorem}
\label{thm: full}
For repeated first-price auctions with budget constraints and full information feedback, \Cref{algo: full} can achieve
\begin{align*}
    Reg(\pi) = O\left(\sqrt{T\ln T}\right).
\end{align*}
\end{theorem}

In the proof of \Cref{thm: full}, we first we perform a standard analysis of the online gradient descent method to show the sequence of $\lambda_t$ is not much worse than a hindsight $\lambda$ with respect to gain function $h_t(\lambda_t) = \lambda_t\left(\widetilde{c}_t(b) - \rho\right)$. This, together with \Cref{lem: full dkw} implies that with high probability, the bid $b_t$ chosen in each round is close to the bid chosen by the best strategy for Problem~\eqref{eqn: soft problem}, i.e., $\arg\max_b (v_t - (1+\lambda^*)b)G(b)$ where $\lambda^*$ is the optimal dual variable. Finally, the proof is concluded by showing that the time at which the budget is depleted under \Cref{algo: full} is close to $T$.

\paragraph{Lower bound.} As previous work has proved, the lower bound on regret for this problem is $\Omega(\sqrt{T})$ even without constraints (i.e., $\rho = \bar{v}$).

\begin{lemma}[\citet{han2020optimal}]
For repeated first-price auctions and full information feedback, there exists a positive constant $C > 0$ independent of $T$ such that
\begin{align}
    \inf_{\pi} \sup_{F, G} Reg(\pi) \geq C\sqrt{T}.
\end{align}
\end{lemma}

This previous result implies that our algorithm can achieve a near-optimal learning performance in first-price auctions with budget constraints.

\paragraph{Discretization.} In \Cref{algo: full}, \Cref{algo: full estimate} requires estimating rewards and costs for all possible bids but the bid space might be continuous. In practice, we can resolve this issue by a simple discretization, which will cause little performance degradation. Let $\calB = \{b^1, \cdots, b^K\}$ with $b^k = (k-1)/K\cdot \bar{v}$. We then change \Cref{algo: full bid} to that the bidder submits a bid
\begin{align}
\label{eqn: best b full quantize}
    b_t \in \arg\max_{b\in \calB} \left(\widetilde{r}_t(v_t, b) - \lambda_t \widetilde{c}_t(b)\right). 
\end{align}
When $K = \Omega(\sqrt{T})$, the discretization error is of order $O(\sqrt{T})$. In the next subsection, we will discretize both values and bids in \Cref{algo: one} and more formally analyze the additional regret caused by the discretization.

==> Budget + FPA (arxiv)/sections/conclusion.tex <==
\section{Conclusion}

In this paper, we study design of bidding algorithms for repeated first-prices auctions with budgets, in both full and one-sided feedback models. On the theoretical side, we prove that \cref{algo: full} can achieve an $\widetilde{O}(\sqrt{T})$ regret in the case with full information feedback and that with a technical assumption \Cref{algo: one} can achieve an $\widetilde{O}(\sqrt{T})$ regret in the case with one-sided information feedback. On the practical side, we show that our algorithms can attain effective budget management as well as good performance. The experiments under different distributions provide evidence that our algorithms can be widely applicable.
%compare the performance of our algorithms to the performance with algorithms proposed in previous work that is near optimal in the problem without constraints. The experiments under distributions that do not satisfy the technical assumption gives evidence that our algorithm can actually be more widely applicable.

%Investigating whether the analysis in this paper can finally hold for any distribution under one-sided information feedback is an open problem worth exploring. 

% If the answer is NO, it is also an interesting future direction to theoretically characterize a class of ``bad'' distributions that will lead to high expect regret.


==> Budget + FPA (arxiv)/sections/experiments.tex <==
\section{Experiments}
\label{sec: exp}

\begin{figure*}[h] 
    \centering
    \begin{subfigure}{0.33\textwidth}
	\centering
	\includegraphics[width=\linewidth]{figures/n-full.pdf}
	\caption{Normal $v_t$ , full feedback.}
	\end{subfigure}
    \begin{subfigure}{0.33\textwidth}
	\centering
	\includegraphics[width=\linewidth]{figures/l-full.pdf}
	\caption{Log-normal $v_t$, full feedback.}
	\end{subfigure}
 \begin{subfigure}{0.33\textwidth}
	\centering
	\includegraphics[width=\linewidth]{figures/u-full.pdf}
	\caption{Uniform $v_t$, full feedback.}
	\end{subfigure}
 \begin{subfigure}{0.33\textwidth}
	\centering
	\includegraphics[width=\linewidth]{figures/n-one.pdf}
	\caption{Normal $v_t$, one-sided feedback.}
	\end{subfigure}
 \begin{subfigure}{0.33\textwidth}
	\centering
	\includegraphics[width=\linewidth]{figures/l-one.pdf}
	\caption{Log-normal $v_t$, one-sided feedback.}
	\end{subfigure}
 \begin{subfigure}{0.33\textwidth}
	\centering
	\includegraphics[width=\linewidth]{figures/u-one.pdf}
	\caption{Uniform $v_t$, one-sided feedback.}
	\end{subfigure}
    \caption{Performance of bidding algorithms with and without budget control, under full \textit{(Upper)} and one-sided \textit{(Lower)} feedback, evaluated with respect to the reward per round. In three columns, private values are respectively sampled from: \textit{(Left)} normal distribution $v_t \sim \mathcal{N}(0.6, 0.1)$, \textit{(Middle)} logarithmic normal distribution $\log v_t \sim \mathcal{N}(-0.4, 0.1)$, and \textit{(Right)} uniform distribution $v_t \sim \mathcal{U}(0.25, 1)$.}%, and restricted to $[0,1]$ as described.}
    \label{fig: 1}
\end{figure*}

In this section, we empirically evaluate the reward obtained by our proposed algorithms with both full and partial information feedback, using data generated from various distributions. The primary objective of the numerical experiments is to demonstrate the effectiveness of budget management in different settings.
%, which can be quickly reproduced for average performance evaluation. 
%In real-world applications, where repeated tests are not needed, better performance may be obtained by more refined yet costly subdivision discretization of bids and values. 
The performance may be further improved by tuning the parameters according to the amount of available budgets. The characterization of such optimal context-dependent parameters is left as an open future problem. 

\paragraph{Setup.} We consider repeated first-price auctions with $T = 10^6$ rounds, budget amount $B = 10^4$ and upper bound on values $\bar{v} = 1$. We generate the sequence of competing bids by sampling each $d_t$ \textit{i.i.d.} from normal distribution $\mathcal{N}(0.4, 0.1)$. 
%To satisfy the prerequisites, for $d_t\not \in [0,1]$, sample another independent value for $d_t$ until it falls in interval $[0,1]$. 
For the sequence of private values, we consider normal distribution, logarithmic normal distribution and uniform distribution respectively.
%all restricted to $[0,1]$ using a similar fashion. 
Detailed parameters of the private value distributions can be found in \Cref{fig: 1}.%For a distribution with cumulative distribution function(CDF) $F$ and non-zero probability mass on interval $I$, then the ``restricted'' distribution has CDF $F_{I}(z) = (F(z)-F(a))/(F(b)-F(a))$. Details of the parallel experiments are elaborated in \Cref{fig: 1}. 

In each experiment, we simulate $T$ rounds auctions under both full and one-sided information structure, and compare our proposed algorithm with ones without budget management, i.e., all the same except for omitting multiplier $\lambda_t$ and using true value $v_t$ instead of $v_t/(1+\lambda_t)$. The performance is evaluated by observing and plotting $\sum_{s=1}^t r_s/t$, the \emph{reward per round} as a function of $t$. For all algorithms, we uniformly set $M = K = 100$, failure probability $\delta = 0.01$, and adopt fixed step size $\epsilon = 1/\sqrt{T}$. For each of the graph we take the average of $20$ independent repetitions of the process.

In the above setup, readers may think $\rho/\bar{v} = 0.01$ is a too tight constraint. However, with an example we show that a seemingly ``tight'' constraint is necessary for budget management to be of even the least use. 
\begin{example}
In $T$-round repeated first price auctions with $v_t, d_t \sim \mathcal{U}(0,1)$, when adopting the optimal strategy for Problem~\eqref{eqn: soft problem}, the soft budget constraint is not binding if $\rho \geq 1/12$.
% under both information structures it takes at least $T$ rounds in expectation for an algorithm without any budget management to deplete its budget. 
\end{example}

We note that the study on budget management is only needed when budget is relatively tight, such as $\rho < 1/12$ in the above example. Otherwise, a bidder can simply ``forget'' $B$, adopt unconstrained strategies, without expecting her budget to run out. %本段也可以考虑放在下面的result and discussion

\paragraph{Results and Discussions.} 
The results of three parallel experiments are plotted in \Cref{fig: 1}, with both full and one-sided information feedback considered. Notably, in all instances, our proposed algorithm outperforms the one with no budget control, with respect to the total reward. The latter algorithm gains remarkable rewards in the beginning rounds, yet tends to deplete its budget in an early phase. The reward per round is then inversely proportional to $t$, and is eventually exceeded by algorithms with budget control. Meanwhile, for algorithms with budget control, the budget can also be depleted in some instances, but only at the very ending phase, with a delicate turning in the tail of each curve. This coincides our argument that the algorithm has its expected time of budget depletion close to $T$. We also note that for the bidding algorithm under one-sided information feedback with budget control, $\sum_{s=1}^t r_s/t$ holds steady in most rounds, which indicates that the algorithm manages to achieve stable per-round gain as the budget is diminishing. This further demonstrates the effectiveness of the proposed algorithms on budget management.

\paragraph{Further Experiments on \Cref{lem: main}.} 
We notice that the proposed algorithm performs well in the third experiment where $v_t \sim \mathcal{U}(0.25, 1)$, which does not satisfies the conditions of \Cref{asm: main}. This indicates that the proposed bidding algorithm with one-sided feedback might perform well on a broader class of private value distributions beyond the requirement of \Cref{asm: main}. The following experiment provides numerical evidence that \Cref{lem: main} is very likely to hold for the value distribution $\mathcal{U}(0.25, 1)$. 

\begin{figure}[h]
    % \centering
    \includegraphics[width=0.9\linewidth]{figures/fig2.pdf}
    \caption{Numerical evidence for \Cref{lem: main} by showing $\mathbb{E} \left[\sum_{t=2}^T ({N_t^{m(t)}})^{-1/2}\right] \leq \sqrt{T\ln T}$, in a case where \Cref{asm: main} does not hold.}
    \label{fig: 2}
\end{figure}

We simulate the bidding algorithm with budget control under one-sided feedback with different time horizons $T = 10^5 \tau$ where $ \tau = 1, \cdots, 10$, while fixing $K = M = 100$. For each horizon $T$, we observe the sequence of values and bids to compute $\sum_{t=2}^T ({N_t^{m(t)}})^{-1/2}$. We repeat the process $10$ times to estimate its expectation, which is compared with $\sqrt{T\ln T}$. The results are plotted in \Cref{fig: 2}.

In \Cref{fig: 2}, the growth rate of the blue curve is notably smaller than $\sqrt{T\ln T}$, supporting the inequality in \Cref{lem: main}. We further conjecture that similar properties may hold for a larger class of distributions, only a subset of which is captured by \Cref{asm: main}. Preciser theoretical characterization of the distribution class is an interesting open problem, which we left as a future direction.

==> Budget + FPA (arxiv)/sections/introduction.tex <==
\section{Introduction}
Recent years have witnessed the explosive growth of the online advertising market. 
It is estimated that worldwide online advertising spending will reach 681 billion dollars in 2023, accounting for nearly 70\% of the entire advertising market spending \cite{adspending2022worldwide}. 
In practice, a huge amount of online ads are sold via real-time auctions implemented on advertising platforms and advertisers participate in such repeated online auctions to purchase advertising opportunities. 
% with the goal of maximizing their targets subject to their specified constraints. 
An advertiser typically aims to maximize her cumulative payoffs during a specific time horizon (e.g., a day or a week) subject to a budget constraint, which reflects her monetary limit throughout this period. The presence of budgets constitutes an important operational challenge for online bidding algorithm design since there will be considerable financial losses whether depleting the budget too early or reaching the end of the period with unused funds. Therefore, budget management is a fundamental issue for designing practical online bidding algorithms. 
% purchase advertising opportunities. Instead of inefficient manual bidding, advertisers are increasingly inclined to online bidding algorithms that determine the bids for incoming queries to maximize advertisers' targets subject to their specified constraints. Thus, designing online bidding algorithms with good performance has become a significant problem in the domain of online advertising.

% An advertiser typically aims to maximize her total utility during a specific time horizon (e.g., a day or a week) subject to a budget constraint, which reflects the advertiser's monetary limit throughout this period. The presence of budgets constitutes an important operational challenge for algorithm design since it interconnects multiple rounds of auctions together. Moreover, there is much uncertainty about future opportunities as advertisers usually have little knowledge about the competition in the online advertising market. These challenges together make it hard for advertisers to balance the present and future advertising opportunities. Whether depleting the budget too early or reaching the end of the period with unused funds, there will be considerable financial losses. Therefore, budget management is a fundamental part of a practical online bidding algorithm.

There has been a flourishing line of literature on budget management strategies in repeated second-price auctions~\cite{balseiro2019learning,balseiro2022best,chen2022dynamic}. 
% The second-price auction was once a prevalent auction mechanism due to its truthful nature \cite{lucking2000vickrey,klemperer2004auctions,lucking2007pennies}. 
However, a major industry-wide shift has occurred recently towards using first-price auctions as the preferred auction format of selling digital ads \cite{despotakis2021first}, as opposed to the earlier prevalent practice of using second-price auctions \cite{lucking2000vickrey,klemperer2004auctions,lucking2007pennies}. Google Ad Exchange, the largest online auction platform, announced its shift to the first-price auction
% for reduced complexity and enhanced transparency
in September 2019~\cite{google2019fpa}. On the one hand, the difference in the nature of first-price auctions and second-price auctions implies that the algorithms proposed by the above work may not directly apply to the first-price setting. On the other hand, most previous work on repeated first-price auctions only considered bidding without budgets \cite{balseiro2019contextual,han2020optimal,han2020learning,badanidiyuru2021learning,zhang2022leveraging}. The shift thus leads to a pressing question of how should an advertiser bid in repeated first-price auctions to maximize the cumulative payoffs while controlling the expenditures. 
% This work answers the question by proposing near-optimal bidding algorithms for repeated first-price auctions with budgets

In this paper, we study the design of online bidding algorithms in repeated first-price auctions with budgets. 
% To answer this question, we need to overcome two challenges:
% \begin{enumerate}
%     \item First, it is known that the strategy in first-price auctions is notoriously complex to analyze, even in the static case \cite{}.
%     \item Second,  usually uses . However, 
% \end{enumerate}
We focus on a \textit{stochastic} setting where both the bidder's values and the maximum competing bids are \textit{i.i.d.} sampled over auctions. 
The goal is to optimize the bidder's expected cumulative rewards while keeping her budget constraint satisfied for any realization of values and competing bids. 
We provide online bidding algorithms for the bidder in two different feedback models: \begin{enumerate*}[label={(\arabic*)}]
    \item the \textit{full information feedback}, where the maximum competing bid is always revealed after each auction;
    \item the \textit{one-sided information feedback}, where only the winning bid is revealed after each auction.
\end{enumerate*}

% \begin{enumerate}
%     \item \textit{Full information feedback.} 
%     The bidder can observe the maximum competing bid at the end of each round. 
%     This information structure makes sense in many current online auction platforms. 
%     For example, in the Google Ad Exchange, at the end of an auction, bidders will receive back the minimum value they would have had to bid to win the auction, whether they lost or won~\cite{google2022adshelp}.
%     \item \textit{One-sided information feedback.} The bidder can observe the maximum competing bid only if she loses the auction. 
%     % Thus, the feedback available to her includes $\mathbbm{1}\{b_t\geq d_t\}$ and $d_t\mathbbm{1}\{b_t < d_t\}$.
%     This can be viewed as an informational version of the \textit{winner’s curse} \cite{capen1971competitive} where the winner learns less information. And this is a common feedback model in previous studies on repeated first-price auctions~\cite{esponda2008information,han2020optimal,ai2022no}. Compared to the full information feedback, the one-sided information feedback is more complicated to deal with as the bidder can observe less information.
% \end{enumerate}

\paragraph{Our Results.} Our main contribution is to propose two near-optimal bidding algorithms for each of the two feedback models. 
For the full information feedback, \Cref{algo: full} can achieve an $\widetilde{O}(\sqrt{T})$ regret where $T$ is the total number of auctions (\cref{thm: full}). 
For the the one-sided information feedback, \Cref{algo: one} can achieve an $\widetilde{O}(\sqrt{T})$ regret under mild assumptions on value distributions (\Cref{thm: one}).

Our algorithms follow a primal-dual framework and update a dual variable via online gradient descent to adjust the rate at which the bidder depletes her budget. The framework is similar to those used by previous work on second-price auctions \cite{balseiro2019learning,balseiro2022best,feng2022online,chen2022dynamic}. However, its application to repeated first-price auctions presents new challenges:
\begin{enumerate}
    \item First, due to the non-truthful nature of first-price auctions, we cannot compute the bid that maximizes the cost-adjusted reward without knowing the highest competing bid. One can only expect to maximize the objective in expectation by learning the hidden distribution of maximum competing bids. However, estimates using historical samples may not be sufficiently accurate. Even worse, with one-sided feedback, the bidder's observations are actually biased.
    % in the case of one-sided information feedback, the This is more difficult in the case with one-sided feedback, where bidder's observations are biased.
    %First, due to the truthful nature of second-price auctions, the primal-dual approach in second-price auctions is able to compute the bid that maximizes the cost-adjusted reward without knowing the maximum competing bid in each round. Since first-price auctions are non-truthful, one can only expect to maximize the cost-adjusted reward in expectation, but the prior distributions of both values and maximum competing bids are unknown to the bidder.
    % it is known that the strategy in first-price auctions is notoriously complex to analyze \cite{lebrun1996existence} so one can only expect to optimize the total rewards in expectation.
    %Estimates using historical samples may not necessarily lead to sufficiently high estimation accuracy, especially for the one-sided information feedback. Even worse, in the case of one-sided information feedback, the bidder's observation of the maximum competing bids is actually biased.
    \item Second, the dynamic update of the dual variable implies that the cost-adjusted reward function differs in different rounds. This causes failure in previous bandit algorithms like \citet{balseiro2019contextual} and \citet{han2020optimal}, as future rounds may suffer from exploitation when objectives are misaligned. %Second, previous work on first-price auctions usually models the problem as a contextual bandit problem and maintains a high-reward action (bid) set for each context (value) \cite{balseiro2019contextual,han2020optimal}. Nevertheless, the dynamic update of the dual variable implies that the cost-adjusted reward differs in different rounds. Given a fixed value, the bid that maximizes the cost-adjusted reward varies to the dual variable. Thus, with the misalignment of objectives, rewards in future rounds may suffer from the arm elimination process (pruning the high-reward action sets) in past rounds.
\end{enumerate}

This work overcomes the two challenges and provides theoretical performance guarantees for our proposed algorithms. 
% For the full information feedback, we combine the online optimization method and the distribution estimation technique to design \Cref{algo: full}. 
% Specifically, we bound the estimation errors of empirical rewards and costs to lower bound the performance. % The algorithm in this setting reveals our high-level idea of budget management in repeated first-price auctions. 
We start with the full information feedback and design \Cref{algo: full}, which sketches the high-level combination of online optimization methods and distribution estimation techniques. 
We then refine the algorithm for the one-sided information feedback, where we introduced value shading (i.e., scaling down the value by a factor) to align the objectives of different rounds so as to balance exploration and exploitation. 
% We maintain a high-reward bid set for each shaded value and leverage the graph-feedback and partial-order properties in first-price auctions, which in essence follows the approach considered in \citet{han2020optimal}. 
% As the bidder's observations are biased in this feedback model, the estimation errors are bounded via a martingale argument.
% For the one-sided information feedback, we use value shading (i.e., scaling down the value by a factor) to align the objectives of different rounds so as to balance the exploration and exploitation. 
We maintain a high-reward bid set for each shaded value and leverage the graph-feedback and partial-order properties in first-price auctions, which in essence follows the approach developed in \citet{han2020optimal}. 
As the bidder's observations are biased in this feedback model, the estimation errors are bounded via a martingale argument. The sum of estimation errors is shown to be upper bounded by $\widetilde{O}(\sqrt{T})$ with an assumption on the bidder's value distribution. In the experimental part, we demonstrate that our algorithms outperform those without budget management under various distributions in terms of the long-run average performance.

% we conduct numerical experiments to demonstrate the effectiveness of our algorithms. The long-run average performance of our algorithms outperforms those without budget management under different distributions, even distributions that do not satisfy our technical assumption.

\subsection{Related Work} 

Learning in repeated auctions with constraints has been extensively studied in literature but most studies focused on only second-price auctions. 
\citet{balseiro2019learning} proposed an optimal online bidding algorithm known as adaptive pacing in repeated second-price auctions with budget constraints. 
% The algorithm shades the bidder's value by a dual variable as her bid in each auction and updates the variable via online gradient descent. 
\citet{balseiro2022best} extended the above work by relaxing some model assumptions and using a more general dual approximation scheme. 
\citet{feng2022online,golrezaei2021bidding} considered repeated second-price auctions with budget and return-on-spend (RoS) constraints.
% \citet{golrezaei2021bidding} considered the same problem but their model only requires the constraints to hold in expectation. 
\citet{chen2022dynamic} studied another important class of budget management strategies, called throttling,
% with which a bidder always report her true values but choose not to enter a fraction of auctions to control the budget. 
and proposed a near-optimal throttling algorithm for repeated second-price auctions with budgets. 
Our work considers budget management in repeated first-price auctions instead but we use some similar techniques to those in the above papers.

For repeated first-price auctions, most previous work only considered bidding without constraints. \citet{balseiro2019contextual} first considered learning in repeated first-price auctions with binary feedback where the bidder only knows whether she wins or not.
% They modeled it as a contextual bandits problem, where the context is the bidder' value and the bidder only knows whether she wins or not.
They adopted a cross-learning approach to achieve an $\widetilde{O}(T^{2/3})$ regret and
% used a reduction to dynamic pricing \cite{kleinberg2003value,cesa2019dynamic} to 
showed that the lower bound on regret
% with binary feedback
is $\Omega(T^{2/3})$. 
\citet{han2020optimal} considered repeated first-price auctions with one-sided feedback, where the winning bid is revealed after each auction. 
They leveraged the graph-feedback and partial-order properties in first-price auctions to achieve an $\widetilde{O}(\sqrt{T})$ regret
% is achievable
% with additional censored feedback of the winning price.
% They also 
and proved that the lower bound on regret
% in repeated first-price auctions
is $\Omega(\sqrt{T})$ even under full information feedback where the maximum competing bid is always revealed after each auction. \citet{han2020learning} considered the setting
% with full information feedback but
without the \textit{i.i.d.} assumption of the maximum competing bids
% assumed by the above models. 
% They 
and achieved an $\widetilde{O}(\sqrt{T})$ regret when competing with the set of all Lipschitz bidding strategies. \citet{badanidiyuru2021learning} studied the contextual first-price auctions where the values and the maximum competing bids depend on a public context. 
\citet{zhang2022leveraging} studied the setting where the bidder has access to some hint relevant to the maximum competing bid.
The main difference between the above papers and ours is that the bidder has a budget constraint in our model.

\citet{ai2022no} also studied no-regret learning in repeated first-prices auctions with budgets. However, their model additionally involves a discount factor $\gamma < 1$ in the objective function and the ``optimal'' strategy is defined with respect to this variant problem. 
% Their algorithm requires solving a set of complex optimization problems in every round, thus unsuitable for the online setting. 
Their algorithm will abort if $\gamma = 1$ so our results are not directly comparable with theirs.

% , which unfortunately makes the total utility at most the sum of a geometric sequence, i.e., a constant independent of $T$. Thus, the $\widetilde{O}(\sqrt{T})$ regret achieved by their algorithm is actually meaningless.

\citet{balseiro2022contextual} studied the equilibrium biding strategies for first-price auctions with budgets. Their value-pacing-based strategies are similar to our second algorithm, but we are investigating a dynamic setting from the view of a single budget-constrained bidder. The equilibrium characterization of the first-price market cannot provide regret guarantees for dynamic bidding, especially considering the learning process with respect to different feedback models.

% \citet{despotakis2021first} explained the rapid and dramatic move from second-price to first-price auction format in the online advertising market by linking the phenomenon to the move from the waterfalling strategy employed by publishers to an alternate header bidding strategy. They argued that given the publisher move to header bidding, exchanges move from second-price to first-price auctions to increase their expected clearing prices.







==> Budget + FPA (arxiv)/sections/preamble.tex <==
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
% \usepackage{subfigure}
%\usepackage{subfig}
\usepackage{booktabs} % for professional tables

\usepackage{bm, bbm}
\usepackage{subcaption, tikz}
\usepackage{multicol, multirow}
\usepackage[inline]{enumitem}

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2023} with \usepackage[nohyperref]{icml2023} above.
\usepackage[hyphens]{url}
\usepackage{hyperref}

\usepackage{float}

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% Use the following line for the initial blind version submitted for review:
% \usepackage{icml2023}

% If accepted, instead use the following line for the camera-ready submission:
\usepackage[accepted]{icml2023}

% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}

% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}
\Crefname{ALC@unique}{Line}{Lines}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{claim}[theorem]{Claim}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{observation}[theorem]{Observation}

% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
\usepackage[textsize=tiny]{todonotes}

\usepackage{xcolor}         % colors
\definecolor{pku-red}{RGB}{139,0,18}

% \usepackage[text=charlie@pku.edu.cn\\Draft\ Copy,scale = 0.5, hpos=0.5\paperwidth,vpos=0.5\paperheight, color={[gray]{0.9}}]{draftwatermark}
\newcommand\wq[1]{\textcolor{pku-red}{[wq: #1]}}

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

\newcommand{\va}{\boldsymbol{a}}
\newcommand{\vb}{\boldsymbol{b}}
\newcommand{\vc}{\boldsymbol{c}}
\newcommand{\vd}{\boldsymbol{d}}
\newcommand{\ve}{\boldsymbol{e}}
\newcommand{\vx}{\boldsymbol{x}}
\newcommand{\vy}{\boldsymbol{y}}
\newcommand{\vz}{\boldsymbol{z}}
\newcommand{\vu}{\boldsymbol{u}}
\newcommand{\vv}{\boldsymbol{v}}
\newcommand{\vw}{\boldsymbol{w}}
\newcommand{\vp}{\boldsymbol{p}}
\newcommand{\vg}{\boldsymbol{g}}

\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bvarepsilon}{\boldsymbol{\varepsilon}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bvartheta}{\boldsymbol{\vartheta}}
\newcommand{\biota}{\boldsymbol{\iota}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}

==> Budget + FPA (arxiv)/sections/preliminaries.tex <==
\section{Model and Benchmark}

% \paragraph{Basic setting.}
In this work, we consider the problem of online learning in the first-price auction market. We focus on a single bidder in a large population of bidders during a time horizon $T$. 

In each round $t = 1, \ldots, T$, there is an available ad slot auctioned by the seller (e.g. an advertising platform). 
The bidder receives a private value $v_t\in [0, \bar{v}]$, and then submits a bid $b_t \in \bbR_+$ based on $v_t$ and all historical observations available to her. 
We denote the maximum bid of all other bidders by $d_t\in \bbR_+$. 
The auction outcome depends on the comparison between $b_t$ and $d_t$. 
Let $x_{t} \coloneqq \bm{1}\left\{b_{t} \geq d_{t}\right\}$ be the binary variable indicating whether the bidder wins the ad slot at round $t$. 
Here we assume that ties are broken in favor of the bidder we concern to simplify exposition. We note that this choice is arbitrary and by no means a limitation of our approach.
Let $r_{t} \coloneqq x_{t}(v_{t} - b_{t})$ be her reward and let $c_{t} \coloneqq x_{t}b_{t}$ be the corresponding cost for a first-price auction.
As usual, we use the bold symbol $\vv$ without subscript $t$ to denote the vector $(v_{1}, \ldots, v_{T})$; the same goes for other variables in the present paper.

The bidder has a budget $B$ that limits the payments she can make over $T$ rounds of auctions, and her maximum expenditure rate is denoted by $\rho \coloneqq B/T$. 
We assume that $\rho \in (0, \bar{v}]$; otherwise, it becomes a problem without constraints as the bidder would never deplete her budget.

We consider a \textit{stochastic} setting where $v_t$ is \textit{i.i.d.} sampled from a distribution $F$ and $d_t$ is \textit{i.i.d.} sampled from a distribution $G$. 
The latter assumption follows from the standard mean-field approximation \cite{iyer2014mean,balseiro2015repeated} and is a common practice in literature. 
The main rationale behind this assumption is that when the number of other bidders is large, on average their valuations and bidding strategies are static over time. 
Note that both $F$ and $G$ are unknown to the bidder.

\paragraph{Information structure.} 
In repeated first-price auctions, the bidder can receive different feedback after each round depending on the information released by the seller. 
In particular, the ability of this bidder to observe the maximum competing bid $d_t$ varies to the information structure. In this paper, we investigate two different information structures:
\begin{enumerate}
    \item \textit{Full information feedback.} 
    The bidder can observe the maximum competing bid $d_t$ at the end of each round $t$. 
    This information structure makes sense in many current online auction platforms. 
    For example, in the Google Ad Exchange, at the end of an auction, bidders will receive back the minimum value they would have had to bid to win the auction, whether they lose or win \cite{google2022adshelp}.
    \item \textit{One-sided information feedback.} The bidder can observe the maximum competing bid $d_t$ only if she loses the auction. 
    Thus, the feedback available to her includes $\bm{1}\{b_t\geq d_t\}$ and $d_t\bm{1}\{b_t < d_t\}$.
    This can be viewed as an informational version of the \textit{winner’s curse} \cite{capen1971competitive} where the winner learns less information. And this is a common feedback model in previous studies on repeated first-price auctions \cite{esponda2008information,han2020optimal,ai2022no}. Compared to the full information feedback, the one-sided information feedback is more complicated to deal with as the bidder can observe less information.
\end{enumerate}

We denote the historical observations available to the bidder before submitting a bid in round $t$ by $\calH_t$. For the full information feedback, we define
\begin{align*}
    % \label{eqn: history full definition}
    \calH^F_t \coloneqq \left(v_{s}, x_{s}, d_{s}\right)_{s=1}^{t-1}.
\end{align*}
At the end of each round $s$, the bidder can append a tuple $(v_{s}, x_{s}, d_{s})$ to the available history. For the one-sided information feedback, we define
% Thus, the feedback available to her includes $\bm{1}\{b_t\geq d_t\}$ and $d_t\bm{1}\{b_t < d_t\}$. We define
\begin{align*}
    % \label{eqn: history one-sided definition}
    \calH^O_t \coloneqq \left(v_{s}, x_{s}, (1-x_s)d_{s}\right)_{s=1}^{t-1}.
\end{align*}
At the end of each round $s$, the bidder knows her value and whether she wins, but the winner can only observe $(1-x_s)d_s = 0$.

\paragraph{Bidding strategy and regret.} A bidding strategy maps $(\calH_t, v_t)$ to a (possibly random) bid $b_t$ for each $t$. We say $\pi$ is \textit{budget feasible} if it generates expenditures that are constrained by the budget for any realizations of values and maximum competing bids, i.e. $\forall \vv, \vd$, 
\begin{align*}
    \sum^T_{t = 1} c^{\pi}_t = \sum^T_{t = 1} \bm{1}\left\{b^{\pi}_t \geq d_t\right\} b^{\pi}_t \leq B = \rho T.
\end{align*}
We denote by $\Pi_0$ the set of all budget feasible strategies. For a strategy $\pi \in \Pi_0$, we denote by $R(\pi)$ the performance of $\pi$, defined as follows:
\begin{align*}
    R(\pi) = & \bbE^{\pi}_{\vv, \vd} \left[\sum_{t=1}^T r^{\pi}_t\right] \\
    = & \bbE^{\pi}_{\vv, \vd} \left[\sum_{t=1}^T \bm{1}\left\{b^{\pi}_{t} \geq d_{t}\right\}\left(v_t - b_t^{\pi}\right)\right],
\end{align*}
where the expectation is taken with respect to the values, the maximum competing bids and any possible randomness embedded in the strategy. The bidder's optimization problem can be written as
\begin{equation}
\label{eqn: problem}
    \begin{aligned}
    \max_{\pi} & \ \bbE^{\pi}_{\vv, \vd} \left[\sum_{t=1}^T \bm{1}\left\{b^{\pi}_{t} \geq d_{t}\right\}\left(v_t - b_t^{\pi}\right)\right] \\
    \text{s.t. } & \ \sum_{t=1}^T \bm{1}\left\{b^{\pi}_{t} \geq d_{t}\right\}b^{\pi}_t \leq \rho T, \ \forall \vv, \vd.
    \end{aligned}
\end{equation}

The regret of the bidder is defined to be the difference in the expected cumulative rewards of the bidder's strategy and the optimal budget feasible bidding strategy, which has the perfect knowledge of $F$ and $G$:
\begin{align*}
    Reg(\pi) = \max_{\pi'\in \Pi_0} R(\pi') - R(\pi).
\end{align*}

% so the optimization problem can be written as
% \begin{equation}
%     \begin{aligned}
%     \max_{\pi} & \ \bbE_{\vv, \vd} \left[\sum_{t=1}^T \bm{1}\left\{b^{\pi}_{t} \geq d_{t}\right\}\left(v_t - b_t^{\pi}\right)\right] \\
%     \text{s.t. } & \ \sum_{t=1}^T \bm{1}\left\{b^{\pi}_{t} \geq d_{t}\right\}b^{\pi}_t \leq \rho T, \ \forall \vv, \vd.
%     \end{aligned}
% \end{equation}

% We denote by $\pi^*$ the optimal strategy that maximizes the cumulative expected rewards subject to the budget constraint:
% \begin{align*}
%     \pi^* = \arg\max_{\pi \in \Pi_0} \sum^T_{t = 1} R^{\pi}_t
% \end{align*}

% The regret of strategy $\pi\in \Pi_0$, denoted by $Reg^{\pi}$, is defined to the difference in the cumulative rewards of strategy $\pi$ and the optimal budget feasible bidding strategy $\pi^*$:
% \begin{align*}
%     Reg^{\pi} = \sum^T_{t = 1} \left(R^{\pi}_t\right)
% \end{align*}

% We assume the bidder aims to maximize her cumulative expected rewards subject to her budget constraint. We consider as 


